Search for anomalous production of prompt same-sign lepton pairs and pair-produced doubly charged Higgs bosons with $\sqrt{s} = 8$ TeV $pp$ collisions using the ATLAS detector

A low-background inclusive search for new physics in events with same-sign dileptons is presented. The search uses proton-proton collisions corresponding to 20.3 fb$^{-1}$ of integrated luminosity taken in 2012 at a centre-of-mass energy of 8 TeV with the ATLAS detector at the LHC. Pairs of isolated leptons with the same electric charge and large transverse momenta of the type $e^{\pm}e^{\pm}, e^{\pm}\mu^{\pm}$, and $\mu^{\pm}\mu^{\pm}$ are selected and their invariant mass distribution is examined. No excess of events above the expected level of Standard Model background is found. The results are used to set upper limits on the cross-sections for processes beyond the Standard Model. Limits are placed as a function of the dilepton invariant mass within a fiducial region corresponding to the signal event selection criteria. Exclusion limits are also derived for a specific model of doubly charged Higgs boson production.

==> Auxiliary.tex <==
%\Large{}
% electron charge flip rate
\begin{figure}[hbt]
\begin{center}
  \includegraphics[width=0.485\columnwidth]{macros/chargemisid/misidrate_datamc.eps}
\caption{Charge misidentification rate as a function of $|\eta|$ for data and MC extracted using the likelihood method. The upper plot shows the misidentification rates while the lower one shows the scale factors which is the ratio between data and MC. The error bars correspond to the fit error.}
\end{center}
\end{figure}
% electron and muon fake factors
\begin{figure}[ht]
\begin{center}
\subfigure[]{
  \includegraphics[width=0.45\columnwidth]{figures/electron_fake_plot.eps}
}
\subfigure[]{
  \includegraphics[width=0.45\columnwidth]{figures/muon_fake_plot.eps}
}
\caption{Factor $f$ used for the estimation of the non-prompt background for (a) electron and (b) muons as a function of \pt. The shaded area corresponds to the statistical and systematic uncertainties added in quadrature.}
\end{center}
\end{figure}

%prompt background control region
\begin{figure}[htbp]
\begin{center}
\subfigure[] {
  \includegraphics[width=0.45\columnwidth]{figures/2isoSS_ee_mll_pr.eps}
}
\subfigure[] {
  \includegraphics[width=0.45\columnwidth]{figures/2isoSS_emu_mll_pr.eps}
}
\subfigure[] {
\includegraphics[width=0.45\columnwidth]{figures/2isoSS_mumu_mll_pr.eps}
}
\caption{Invariant mass distributions of isolated (a) $ee$, (b) $e\mu$, and (c, d) $\mu \mu$ pairs in the prompt background control region. This region is mainly composed of $WZ$ and $ZZ$ events and contain events with at least a same-flavour opposite-sign pair with invariant mass ($m_{\mathrm{\ell \ell }}$) $|m_{\mathrm{\ell \ell}} - m_{\mathrm{Z}}| < 10$ \gev. The contributions from the various physics processes are shown. The lower plots show the ratio of pairs found in data compared to the SM predictions. The error bars on the data points show the statistical uncertainty and the dashed band shows the statistical and systematic uncertainties added in quadrature of the predictions. The last bin in the histograms includes overflows and is normalised as though it is 50 \gev\ wide.}
\end{center}
\end{figure}
% Electron charge flip control region
\begin{figure}[htbp]
\begin{center}
\includegraphics[width=0.6\columnwidth]{figures/2isoSS_ee_mll_ssz.eps}
\caption{Distribution of the invariant mass of the electron pair, in the same-sign \Zboson\ peak control region. To test the prediction of charge misidentification two isolated electrons with the same charge whose mass is compatible with a $Z$ boson (defined as $80 < m_{\mathrm{ee}} < 100$ \gev) are requested.
The lower plots show the ratio of data over the background prediction. The error bars on the data points show the statistical uncertainty and the dashed band shows the statistical and systematic uncertainties added in quadrature of the predictions.
}
\end{center}
\end{figure}
%
% signal region pt plots
\begin{figure}[htbp]
\begin{center}
\subfigure[]{\includegraphics[width=0.42\columnwidth]{figures/2isoSS_ee_pt1.eps} }
\subfigure[]{\includegraphics[width=0.42\columnwidth]{figures/2isoSS_ee_eta1.eps} }
\subfigure[]{\includegraphics[width=0.42\columnwidth]{figures/2isoSS_emu_pt1.eps} }
\subfigure[]{\includegraphics[width=0.42\columnwidth]{figures/2isoSS_emu_eta1.eps} }
\subfigure[]{\includegraphics[width=0.42\columnwidth]{figures/2isoSS_mumu_pt1.eps} }
\subfigure[]{\includegraphics[width=0.42\columnwidth]{figures/2isoSS_mumu_eta1.eps} }
\caption{(a) \pt\ and (b) pseudorapidity distribution of the leading lepton in the \ee\ channel in the same-sign signal region. Figures (c) and (d) show similar plots for the \emu\ channel and (e) and (f) for the \mumu\ channel. 
  The error bars on the data points show the statistical uncertainty and the dashed band shows the total uncertainties of the predictions. The total uncertainties are the statistical and systematic uncertainties added in quadrature. The last bin in the histograms (a), (c) and (e) includes overflows and is normalised as though it is 20 \gev\ wide.}
\end{center}
\end{figure}
%
% signal region with DCH signals
\begin{figure}[thbp]
\begin{center}
\subfigure[]{\includegraphics[width=0.47\columnwidth]{figures/2isoSS_ee_mll_dch.eps} }
\subfigure[]{\includegraphics[width=0.47\columnwidth]{figures/2isoSS_emu_mll_dch.eps} }
\subfigure[]{\includegraphics[width=0.47\columnwidth]{figures/2isoSS_mumu_mll_dch.eps} }
\caption{\label{fig:dileptonmassDCH} Invariant mass distribution of (a) \ee\ (b) \emu\ and (c) \mumu\ pairs as a function of the dilepton mass in the same-sign signal region. The mass range between 70~\gev\ and 110~\gev\ is not shown in the \ee\ channel as this region is used to estimate the background from charge misidentification. 
Doubly charged Higgs signals are also plotted on top of expected backgrounds.
The error bars on the data points show the statistical uncertainty.
The last bin in the histograms includes overflows and is normalised as though it is 50 \gev\ wide.}
\end{center}
\end{figure}
%
%Event Displays
\begin{figure}[htbp]
\begin{center}
\subfigure[] {
  \includegraphics[width=0.6\columnwidth]{figures/combined_ee.eps}
}
\subfigure[] {
\includegraphics[width=0.6\columnwidth]{figures/combined_emu.eps}
}
\subfigure[] {
\includegraphics[width=0.6\columnwidth]{figures/EventDisplays/combined_mumu.eps}
}
\caption{Event displays for some of the same-sign dilepton pairs with the highest invariant mass in the 2012 data. Here the magenta cones represent electrons which pass the signal selection criteria; the red tracks depict muons which pass the signal selection criteria; the blue boxes depict hits in the muon spectrometers; the green and yellow boxes display projections of the electromagnetic calorimeter energy depositions and the orange tracks are charged particles in the inner detector (shown as a transparent blue cylinder). The event shown in (a) contains a $e^+e^+$ pair with a mass of 964 \gev. The leading (subleading) electron has $\pt = 145~(131)$~\gev, $\eta = -1.7~(2.2)$ and $\phi = 1.9~(-1.3)$. The event in (b) contains a $e^- \mu^-$ pair with a mass of 736 \gev. The electron (muon) has $\pt = 204~(282)$~\gev, $\eta = 0.0~(-2.0)$ and $\phi = 2.7~(-0.4)$. The event in (c) contains a $\mu^- \mu^-$ pair with a mass of 628 \gev. The leading (subleading) muon has $\pt = 154~(133)$~\gev, $\eta = -0.8~(2.0)$ and $\phi = 3.0~(-0.2)$.}
\end{center}
\end{figure}


